Stability of P2P Networks Under Greedy Peering (Full Version)

Major cryptocurrency networks have relied on random peering choice rules for making connections in their peer-to-peer networks. Generally, these choices have good properties, particularly for open, permissionless networks. Random peering choices however do not take into account that some actors may choose to optimize who they connect to such that they are quicker to hear about information being propagated in the network. In this paper, we explore the dynamics of such greedy strategies. We study a model in which nodes select peers with the objective of minimizing their average distance to a designated subset of nodes in the network, and consider the impact of several factors including the peer selection process, degree constraints, and the size of the designated subset. The latter is particularly interesting in the context of blockchain networks as generally only a subset of nodes are the propagation source for content. We first analyze an idealized version of the game where each node has full knowledge of the current network and aims to select the $d$ best connections, and prove the existence of equilibria under various model assumptions. Since in reality nodes only have local knowledge based on their peers' behavior, we also study a greedy protocol which runs in rounds, with each node replacing its worst-performing edge with a new random edge. We exactly characterize stability properties of networks that evolve with this peering rule and derive regimes where stability is possible and even inevitable. We also run extensive simulations with this peering rule examining both how the network evolves and how different network parameters affect the stability properties of the network. Our findings generally show that the only stable networks that arise from greedy peering choices are low-diameter and result in disparate performance for nodes in the network.

==> figures/graph1.tex <==
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,213); %set diagram left start at 0, and has height of 213
%Flowchart: Connector [id:dp3868600800691293] 
\draw   (195,53.25) .. controls (195,40.69) and (205.52,30.5) .. (218.5,30.5) .. controls (231.48,30.5) and (242,40.69) .. (242,53.25) .. controls (242,65.81) and (231.48,76) .. (218.5,76) .. controls (205.52,76) and (195,65.81) .. (195,53.25) -- cycle ;
%Flowchart: Connector [id:dp7783566489155551] 
\draw   (305,172.25) .. controls (305,159.69) and (315.52,149.5) .. (328.5,149.5) .. controls (341.48,149.5) and (352,159.69) .. (352,172.25) .. controls (352,184.81) and (341.48,195) .. (328.5,195) .. controls (315.52,195) and (305,184.81) .. (305,172.25) -- cycle ;
%Flowchart: Connector [id:dp829717883015476] 
\draw   (195,177.25) .. controls (195,164.69) and (205.52,154.5) .. (218.5,154.5) .. controls (231.48,154.5) and (242,164.69) .. (242,177.25) .. controls (242,189.81) and (231.48,200) .. (218.5,200) .. controls (205.52,200) and (195,189.81) .. (195,177.25) -- cycle ;
%Flowchart: Connector [id:dp08137888401490223] 
\draw   (305,50.25) .. controls (305,37.69) and (315.52,27.5) .. (328.5,27.5) .. controls (341.48,27.5) and (352,37.69) .. (352,50.25) .. controls (352,62.81) and (341.48,73) .. (328.5,73) .. controls (315.52,73) and (305,62.81) .. (305,50.25) -- cycle ;
%Straight Lines [id:da450528699883888] 
\draw    (218.5,76) -- (218.5,152.5) ;
\draw [shift={(218.5,154.5)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7804114099662839] 
\draw    (218.5,76) -- (326.84,148.39) ;
\draw [shift={(328.5,149.5)}, rotate = 213.75] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da6739206463303767] 
\draw    (328.5,73) -- (220.11,153.31) ;
\draw [shift={(218.5,154.5)}, rotate = 323.46] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da43701337224323034] 
\draw    (328.5,73) -- (328.5,147.5) ;
\draw [shift={(328.5,149.5)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da6360234467286516] 
\draw    (305,172.25) -- (240.5,174.43) ;
\draw [shift={(238.5,174.5)}, rotate = 358.06] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;


% Text Node
\draw (221.5,48.25) node   [align=left] {\begin{minipage}[lt]{21.08pt}\setlength\topsep{0pt}
$\displaystyle m_{1}$
\end{minipage}};
% Text Node
\draw (336,47.75) node   [align=left] {\begin{minipage}[lt]{24.48pt}\setlength\topsep{0pt}
$\displaystyle m_{2}$
\end{minipage}};
% Text Node
\draw (221.5,171.25) node   [align=left] {\begin{minipage}[lt]{21.08pt}\setlength\topsep{0pt}
$\displaystyle m_{3}$
\end{minipage}};
% Text Node
\draw (332.5,168.25) node   [align=left] {\begin{minipage}[lt]{21.08pt}\setlength\topsep{0pt}
$\displaystyle m_{4}$
\end{minipage}};


\end{tikzpicture}

==> figures/graph2.tex <==
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,213); %set diagram left start at 0, and has height of 213

%Shape: Rectangle [id:dp4480694219447804] 
\draw   (441,32.5) -- (511,32.5) -- (511,180) -- (441,180) -- cycle ;
%Curve Lines [id:da3102936873566472] 
\draw    (496,88.5) .. controls (554.71,27.8) and (586.68,136.4) .. (498.34,109.91) ;
\draw [shift={(497,109.5)}, rotate = 17.28] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp04513011644135578] 
\draw   (235,29.5) -- (305,29.5) -- (305,177) -- (235,177) -- cycle ;
%Straight Lines [id:da9093204401566072] 
\draw    (305,97.5) -- (432.16,43.28) ;
\draw [shift={(434,42.5)}, rotate = 156.91] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da5658805206462475] 
\draw    (305,97.5) -- (439,100.46) ;
\draw [shift={(441,100.5)}, rotate = 181.26] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9087556850534083] 
\draw    (305,97.5) -- (433.21,161.61) ;
\draw [shift={(435,162.5)}, rotate = 206.57] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (478,23) node   [align=left] {\begin{minipage}[lt]{68pt}\setlength\topsep{0pt}
$\displaystyle d-1\ miners$
\end{minipage}};
% Text Node
\draw (606,89) node   [align=left] {\begin{minipage}[lt]{68pt}\setlength\topsep{0pt}
$\displaystyle  \begin{array}{{>{\displaystyle}l}}
edges\ in\ this\ group\\
\ form\ a\ clique
\end{array}$
\end{minipage}};
% Text Node
\draw (276.5,91.25) node  [font=\Large] [align=left] {\begin{minipage}[lt]{25.16pt}\setlength\topsep{0pt}
A
\end{minipage}};
% Text Node
\draw (478.5,89.75) node  [font=\Large] [align=left] {\begin{minipage}[lt]{25.16pt}\setlength\topsep{0pt}
B
\end{minipage}};
% Text Node
\draw (280,20) node   [align=left] {\begin{minipage}[lt]{68pt}\setlength\topsep{0pt}
$\displaystyle m-( d-1) \ $
\end{minipage}};


\end{tikzpicture}


==> figures/graph3.tex <==
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,213); %set diagram left start at 0, and has height of 213

%Shape: Rectangle [id:dp4480694219447804] 
\draw   (441,32.5) -- (511,32.5) -- (511,180) -- (441,180) -- cycle ;
%Shape: Rectangle [id:dp04513011644135578] 
\draw   (235,29.5) -- (305,29.5) -- (305,177) -- (235,177) -- cycle ;
%Straight Lines [id:da9093204401566072] 
\draw    (305,97.5) -- (432.16,43.28) ;
\draw [shift={(434,42.5)}, rotate = 156.91] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da5658805206462475] 
\draw    (305,97.5) -- (439,100.46) ;
\draw [shift={(441,100.5)}, rotate = 181.26] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9087556850534083] 
\draw    (305,97.5) -- (433.21,161.61) ;
\draw [shift={(435,162.5)}, rotate = 206.57] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (493.5,20) node   [align=left] {\begin{minipage}[lt]{104.04pt}\setlength\topsep{0pt}
$\displaystyle d-1\ \ non-miners$
\end{minipage}};
% Text Node
\draw (276.5,97.25) node  [font=\Large] [align=left] {\begin{minipage}[lt]{25.16pt}\setlength\topsep{0pt}
A
\end{minipage}};
% Text Node
\draw (483.5,100.75) node  [font=\Large] [align=left] {\begin{minipage}[lt]{25.16pt}\setlength\topsep{0pt}
B
\end{minipage}};
% Text Node
\draw (270,15.75) node   [align=left] {\begin{minipage}[lt]{44.88pt}\setlength\topsep{0pt}
$\displaystyle d\ miners$
\end{minipage}};


\end{tikzpicture}



==> ideal.tex <==
\newcommand{\game}{{\mathcal G}}
\newcommand{\score}{{score_G}}
\newcommand{\junk}[1]{}
\section{An idealized game-theoretic model}
We consider first an idealized game-theoretic model with $n$ nodes and $m \le n$ miners in which each node wants to select their outgoing peers so as to minimize the average distance to a miner.  A natural approach is via the concept of Nash equilibrium.  Let $d_{out}$ denote the out-degree of each node.  For a given node $v$, an action is a set of at most $d_{out}$ nodes of the network representing the out-neighbors that $v$ selects.  A crucial point to note is that while we distinguish between in- and out-edges, the distances among nodes and the average diameter are based on the graph that is obtained by viewing each edge as undirected.  

Let $\game(n,m,d_{out})$ denote the game with $n$ nodes, $m$ miners, out-degree $d_{out}$, and no bounds on in-degree.  We first show that this game always has a pure Nash equilibrium, a stable topology in which no node wants to change its out-neighbors.

\begin{lemma}
For all $n, m, d_{out}$, $\game(n,m,d_{out})$ has a Nash equilibrium.
\end{lemma}
\begin{proof}
Consider any graph $G$ with the following properties: (i) there exists a node $r$ such that every node in $G$ has an edge to $r$; (ii) every edge is directed to a miner; (iii) there does not exist any pair of nodes $u$ and $v$ such that $(u,v)$ and $(v,u)$ are both present in $G$; and (iv) if a node $v$ has less than $d_{out}$ outgoing edges, then it has an edge to or from every miner.

We claim that $G$ is a Nash equilibrium.  We compute the score for each node in $G$.  We consider miner $r$; $\score{r}$ equals $(m-1)/m$ since every other miner is at distance 1; this is the lowest score possible and no action of $r$ can improve it.  Let $u \neq r$ denote any other miner, and let $i_u$ denote the number of miners that are edges to $u$.  Since $r$ is adjacent to every other node, $u$ is at distance at most $2$ from any other miner.  Given the choices of all other nodes, a best-response action of $u$ is to set all its out-edges to miners that do not have an edge to $u$; the best score achievable equals $\max\{(d_{out} + i_u) + 2(m-i_u-d_{out}), (m-1)\}/m$.  This is precisely what is achieved in $G$ given the conditions: by (ii), all edges are directed to a miner; by (iii) $u$ does not put any out-edges to a miner that already has an edge to $u$; finally, by (iv), if $u$ does not use all of its $d_{out}$ edges, then it already has a score of $(m-1)/m$.

We finally consider a non-miner $v$.  By the conditions, all of the edges of a non-miner are to miners.  Its distance to $\min\{d_{out}, m\}$ miners is 1 and its distance to every other miner is 2, leading to an optimal possible score of $\max\{(d_out + 2(m-d_{out}))/m$.  Thus, $v$ has no incentive to change its out-edges.  We have thus shown that $G$ is a pure Nash equilibrium.
\end{proof}

We next consider the network formation game with a cap on the in-degree.  For concreteness, we consider $d_{in} = 2d_{out}$.  Since the endpoints of the out-edges are constrained by the in-degree cap, reasoning about stable networks is much more challenging.  We first show that $\game(n, m, 1, 2)$ has a pure Nash equilibrium for infinitely many choices of $n$ and $m$.

\begin{lemma}
For any $n = 3\cdot 2^k$ and $m = 3\cdot 2^{k'}$ for any integers $k$, $k'$, $k \ge k' \ge 0$, $\game(n, m, 1, 2)$ has a pure Nash equilibrium.
\end{lemma}
\begin{proof}
Note that $n$ and $m$ are at least 3.  Let $C$ be a directed triangle over three miners $v_1$, $v_2$, and $v_3$.  Partition the remaining nodes into three equal-sized sets $S_1$, $S_2$, and $S_3$.  By the assumption on $n$, each $S_i$ has $2^k - 1$ nodes and $2^{k'}-1$ miners.  Let $T_i$ denote a balanced complete binary directed tree over $S_i$, with every edge directed to the parent, for $1 \le i \le 3$.  Furthermore, assume that the all nodes in $T_i$ with a path to root of length at most $k'-1$ are miners (there are exactly $2^{k'}-1$ such nodes).  Let $r_i$ denote the root of $T_i$.  Consider the network $G$ consisting of the union of $C$, $T_1$, $T_2$, $T_3$, and the edges $\{(r_i, v_i): 1 \le i \le 3\}$.  We show that $G$ is a pure Nash equilibrium.

We first argue that for any leaf $\ell$ and any non-leaf node $v$, the score of $\ell$ is at least the score of $v$.  {\bf Fill the argument here.}

To complete the proof, we consider each node and verify that their out-edge in $G$ gives the node the best score, given the choices of other nodes.  By construction, every non-leaf node in $G$ has an in-degree of 2.  Hence, the action of any node $v$ in the game is to either to have their out-edge in $G$ or to one of the leaf nodes.  If the node $v$ selects a leaf node $\ell$ to be its out-neighbor, then the new score of $v$ would be $(n \cdot s + (n-2))/n \le s$, which would be worse than the current score of $v$.  Hence, the out-edge of $v$ in $G$ is indeed the best-response of $v$ in the game.  This completes the proof that $G$ is a pure Nash equilibrium. 
\end{proof}


Our next result that the network formation game with a cap on the in-degree need not have a pure Nash equilibrium.  In fact, we establish this for one of the simplest cases when $d_{out}$ is $1$ and $d_{in}$ is 2.

\begin{lemma}
For every $n \ge 10$, $\game(n,n,1,2)$ does not have any pure Nash equilibrium.
\end{lemma}
\begin{proof}
Consider any directed graph $G$ with out-degree 1 and in-degree at most 2 for each node.  We first argue that if the undirected version of $G$ is not connected, then $G$ cannot be stable.  For the sake of contradiction, suppose there are two connected components $G_1$ and $G_2$ in the undirected version of $G$.  Since the degree of every vertex is 1, there must be a vertex $v$ in $G_1$ that has at least one incoming edge; then $v$ can improve its score by setting its outgoing edge to a node in $G_2$, increasing the number of nodes to which its distance is finite.

In the remainder, we assume that the undirected version of $G$ is connected.  We next observe that there is a directed cycle in $G$.  We find such a directed cycle by doing a directed walk starting from an arbitrary node $v_0$ and repeatedly following the lone out-edge of the current node.  Let $v_i$ denote the unique out-neighbor of $v_{i-1}$ for $i \ge 1$.  Since there is a finite number of nodes, the walk will visit a node twice.  Let $v_j = v_k$, $j < k$ be the first node visited twice.  Then, $v_j \rightarrow v_{j+1} \ldots v_{k-1} \rightarrow v_k$ is a directed cycle; let us label it $C$.

Each node in $C$ can have at most one incoming edge from outside $C$.  Let $k$ be the number of such nodes.  Consider the graph $G'$ obtained by removing $C$ and the $k$ edges incoming to $C$.  This results in $k$ directed graphs $T_1$ through $T_k$ that have no edges among one another.  Since the total number of edges is $n$, it follows that the number of edges in $T_1$ through $T_k$ is $n - |C| - k$; since $n - |C|$ is the number of nodes in $T_1$ through $T_k$, it follows that each $T_i$ is an root-ward directed tree with its root having an edge to a node in $C$.

Let $\ell$ be a leaf in $T_i$.  Clearly, its score equals $(n s + n - 2)/n$, where 
\end{proof}

==> sections/app_additional_plots.tex <==
\section{Additional plots}


    \subsection{In-bound cap}
     \label{app:in-cap}
     \begin{figure}[H]
            \centering
            \begin{subfigure}{.75\textwidth}
                \centering
                \includegraphics[width=\linewidth]{figures/perigee-sim/100-100-net-diam-mult.png}
               % \caption{Network Diameter All Miners}
            \end{subfigure}\\
            \begin{subfigure}{.75\textwidth}
                \centering
                \includegraphics[width=\linewidth]{figures/perigee-sim/100-10-net-diam-mult.png}
                %\caption{Network Diameter $m=10$}
            \end{subfigure}\\
            \begin{subfigure}{.75\textwidth}
                \centering
                \includegraphics[width=\linewidth]{figures/perigee-sim/100-10-min-diam-mult.png}
                %\caption{Miners Diameter $m=10$}
            \end{subfigure}
            \caption{Diameter of a 100 node network with all miners and a subset of 10 miners, and the diameter between the 10 miners. }
            \label{fig:mult-diam}
    \end{figure}


    \subsection{Network size}
    \label{app:network-size}
    \begin{figure}[H]
            \centering
            \begin{subfigure}{.45\textwidth}
                \centering
                \includegraphics[width=\linewidth]{figures/perigee-sim/100-10-diam.png}
                \caption{100 nodes diameter}
            \end{subfigure}
            \begin{subfigure}{.45\textwidth}
                \centering
                \includegraphics[width=\linewidth]{figures/perigee-sim/100-10-eccen.png}
                \caption{100 nodes eccentricity}
            \end{subfigure}\\
            \begin{subfigure}{.45\textwidth}
                \centering
                \includegraphics[width=\linewidth]{figures/perigee-sim/400-10-diam.png}
                \caption{400 nodes diameter}
            \end{subfigure}
            \begin{subfigure}{.45\textwidth}
                \centering
                \includegraphics[width=\linewidth]{figures/perigee-sim/400-10-eccen.png}
                \caption{400 nodes eccentricity}
            \end{subfigure}\\
            \begin{subfigure}{.45\textwidth}
                \centering
                \includegraphics[width=\linewidth]{figures/perigee-sim/900-10-diam.png}
                \caption{900 nodes diameter}
            \end{subfigure}
            \begin{subfigure}{.45\textwidth}
                \centering
                \includegraphics[width=\linewidth]{figures/perigee-sim/900-10-eccen.png}
                \caption{900 nodes eccentricity}
            \end{subfigure}
            \caption{Diameter and eccentricity over time for networks of 100, 400, and 900 nodes with 10 miners and out-degree 10. Evidence miners are mostly finding each other, it just takes some time for a clique to form.}
            \label{fig:10-diam-eccen}
    \end{figure}
    

    \subsection{K-worst edges}
        \label{app:kworst}

    \begin{figure}[H]
            \centering
            \begin{subfigure}{.45\textwidth}
                \centering
                \includegraphics[width=\linewidth]{figures/perigee-sim/100-10-din-ks.png}
                \caption{capped}
            \end{subfigure}
            \begin{subfigure}{.45\textwidth}
                \centering
                \includegraphics[width=\linewidth]{figures/perigee-sim/100-10-uncap-din-ks.png}
                \caption{uncapped}
            \end{subfigure}
            \caption{In-degree distribution for different $k$-worst values for sub-network of miners. The case when all nodes are miners looks the same. For the capped case, the larger the $k$, the closer the network behaves to the initial random graph.}
            \label{fig:din-ks}
    \end{figure}

    \begin{figure}[H]
            \centering
            \begin{subfigure}{.75\textwidth}
                \centering
                \includegraphics[width=\linewidth]{figures/perigee-sim/100-100-diam-net-ks.png}
                %\caption{network diameter all miners }
            \end{subfigure}
            \begin{subfigure}{.75\textwidth}
                \centering
                \includegraphics[width=\linewidth]{figures/perigee-sim/100-10-diam-net-ks.png}
                %\caption{network diameter 10 miners}
            \end{subfigure}
            \begin{subfigure}{.75\textwidth}
                \centering
                \includegraphics[width=\linewidth]{figures/perigee-sim/100-10-diam-min-ks.png}
                %\caption{miner diameter 10 miners}
            \end{subfigure}
            \caption{Network diameter for all miners, subset miners and miner diameter for subset miners for different $k$-worst values. All three plots are for uncapped $d_{in}$, when $d_{in}$ is capped the network diameter is constant. We see the network diameter is generally approaching 2, and that higher $k$ leads to quicker convergence. Interestingly, the miner diameter is minimal at $k=3$.}
            \label{fig:diam-ks}
    \end{figure}
    

    

 




==> sections/app_full_proofs.tex <==
\section{Full proofs}

    \subsection{Proofs of Lemma~\ref{lem:nash-capped} and~\ref{lem:nash_capped_general}}
    \label{app:nash-capped}
    \begin{lem}[Stable Networks in Capped Games with Unit Out-Degree]
        For any $n = 3\cdot d^k$ and $m = 3\cdot d^{k'}$ for any integers $k$, $k'$, $k \ge k' \ge 0$, $\game(n, m, 1, d)$ has a pure Nash equilibrium.
    \end{lem}
    \begin{proof}
        Note that $n$ and $m$ are at least 3. Let $C$ be a directed triangle over three miners $v_1$, $v_2$, and $v_3$.  Partition the remaining nodes into three equal-sized sets $S_1$, $S_2$, and $S_3$.  By the assumption on $n$, each $S_i$ has $d_{in}^k - 1$ nodes and $d_{in}^{k'}-1$ miners.  Split each $S_i$ into $d_{in}-1$ balanced complete $d_{in}$-ary directed trees, with every edge directed to the parent.
        Note that a balanced complete $d_{in}$-ary tree of depth $h-1$ has $\frac{d_{in}^h-1}{d_{in}-1}$ nodes. Furthermore, assume that all nodes in each $d_{in}$-ary tree $T_j$ up to depth $k'-1$ are miners (there are exactly $\frac{d_{in}^{k'}-1}{d_{in}-1}$ such nodes in each $T_j$). Let $r_{i,j}$ for $1\le j \le d_{in}-1$ be the root of each tree $T_j$ in $S_i$. Consider the network $G$ consisting of the union of $C$, $S_1$, $S_2$, $S_3$, and the edges $\{(r_{i,j}, v_i): 1 \le i \le 3\}$.  We show that $G$ is a pure Nash equilibrium.
    
        For each $v_i$, consider the directed tree $Tv_i$ made up of the trees in $S_i$ and the edges from their roots to $v_i$. By symmetry, the scores of all nodes at a given depth in $Tv_i$ are the same. Let $\delta_1$ and $\delta_2$ be integers such that $k \ge \delta_1 > \delta_2$. Consider two nodes $n_1$ and $n_2$ in $S_i$ at depths $\delta_1$ and $\delta_2$, respectively.  The score of $n_1$ is strictly greater than that of $n_2$. This is because a node $v$ at some depth $\delta$ has a lower score than any of the nodes in the sub-tree below it since there are twice as many miners not in $Tv_i$ as are in $Tv_i$, and $v$ is in the only path of its sub-tree to those miners. This also implies that for any leaf $\ell$ and any non-leaf node $v$, the score of $\ell$ is at least the score of $v$. Given the symmetry of the leaves, this applies for all $n_1,n_2$ at depths $\delta_1$ and $\delta_2$ in different $Tv_i$ trees. 
    
        To complete the proof, we consider each node and verify that their out-edge in $G$ gives the node the best score, given the choices of other nodes.  By construction, every non-leaf node in $G$ has a full in-degree of $d$.  Hence, the action of any node $v$ in the game is to either have their current out-edge in $G$ or to direct the out-edge to one of the leaf nodes. If $v$ selects a leaf node $\ell$, note that by symmetry this node has score $s$ at least that of $v$. If $v$ is not a miner, then its distance to all miners will be one more than that of $\ell$, so the new score of $v$ is $s+1$. 
    
        If $v$ is a miner at depth $h$, we consider the change in its score as new\_score$(v)-$old\_score$(v)$ and prove this change is positive. Note first that $v$'s distance to itself and all miners in the sub-trees that point to $v$ remains the same, so a difference of 0. WLOG, assume $v$ was in $Tv_1$ and chose to connect to a leaf in $Tv_2$. Thus $v$'s distance to miners in $Tv_3$  has only increased by $k+1-h$.    
        %, thus the change in cumulative distance for $Tv_3$ is $(k+1-i)\cdot d^{k'}$. 
        Next, let $v'$ be the new ancestor of $v$ in $Tv_2$ at height $h$. Since $v$ and $v'$ were at the same height in $G$, by the symmetric property of $G$, they had the same cumulative distance to miners in $Tv_1$ and $Tv_2$ who are not in the sub-trees of $v$ or $v'$. Thus $v$'s score to these miners has increased by its distance to $v'$ which is again $k+1-h$.
        %, thus the change in cumulative distance for these miners is $(k+1-i) \cdot 2 \cdot (d^{k'}-\frac{d^{k'-i+1}-1}{d-1})$.
        
        The only remaining miners to consider in the change in score is from $v$ to the miners in the sub-tree of $v'$ which may now be closer (i.e., take away from the change in score). In the original structure, $v$ was a maximum $2h+1$ from $v'$ ($2h$ if $v$ and $v'$ are in the same tree), thus these miners are now at most $k+h+1$ from $v$. If we consider only the sub-trees of $G$ whose roots are at depth $h$, let $X$ be the number of miners in each of these sub-trees. There are $(d-1)*d^{h-1}$ such sub-trees in each $S_i$. Then new\_score$(v)-$old\_score$(v)$ is at least the score difference for these sub-trees (since we are just under-counting miners who are now further away from $v$), we get that 
        %
        $$ \text{new}\_\text{score}(v)-\text{old}\_\text{score}(v) \geq (k+1-h)\cdot \left[ 3 \cdot (d-1)\cdot d^{h-1} -2 \right]\cdot X  - (k+h+1)\cdot X.$$ 
        %
        Let's assume this score difference is non-positive. Remembering that  $d\geq 2$, we can simplify the above inequality to be 
        %
        $$2^{h-1}\leq (d-1)d^{h-1}\leq \frac{3k+h-3}{3k-3h+3}$$
        %
        which is not satisfiable. Thus the score difference is strictly positive, meaning $v$ would not choose to change its out-edge.
    \end{proof}

\begin{lem}[Stable Networks in Capped Games with Arbitrary Out-Degree]
For integers $k \ge 0$, $d \ge 2$, $m = 2^k$, and $n \ge 2^{3k}$,   $\game(n, m, d, 2d)$ has a pure Nash equilibrium.
\end{lem}
\begin{proof}
  We consider a network $G$ that has three components. The first component $G_1$ is a graph with its vertex set being all the miners, each node with an out-degree of $d$ to other miners, leaving $d2^k$ incoming capacity. 
  
  The second component $G_2$ consists of $k+1$ levels of nodes, with level $i \ge 0$ consisting of set $L_i$ of $2^{k+i}$ nodes.  For each $i$, we partition the $2^{k+i}$ nodes into $2^{i}$ groups of $2^k$ nodes each; we label these groups $S_{i,0}, \ldots, S_{i,2^{i+1}-1}$.
  For any non-negative integer $j_{k-1} < 2^{k}$, the node groups $S_{i,j_i}$, $j_i = \lfloor j_{i+1}/2 \rfloor$, $-1 \le i < k$, include a butterfly network.  That is, 
  the edges between $S_{i,j_i}$ and $S_{i+1,j_{i+1}}$, with $j_i = \lfloor j_{i+1}/2 \rfloor$ include the $i$th level of an $2^k$-input butterfly network.  This can be set up since $d \ge 2$. 
  This ensures that every node in $L_{k}$ has a path of length $k$ to every node in $S_{1, 0}$.   (Instead of using a butterfly network, we could also have random biregular bipartite graphs between consecutive levels, achieving the same distance property between $L_{k}$ and $S_{1,0}$ with high probability.) We can then place all remaining edges from each $L_i$ arbitrarily to nodes in $L_{i-1}$. We then have all edges from $S_{1,0}$ go into $G_1$, thus all nodes at level $L_{k}$ have the same score as all their paths to the miners converge at $L_0$.

  %There is a random bipartite graph with $d$ outgoing edges from each node in $L_0$ and $2d$ incoming edges into each of the $m/2$ nodes in $G_1$ with zero in-degree in $G_1$. 
 %For each $i > 0$, there is a random bipartite graph connecting $L_i$ to $L_{i-1}$ with $d$ outgoing edges for each node in $L_i$ and $2d$ incoming edges for each node in $L_{i-1}$. 

 The final component $G_3$ consists of at least $k$ levels of nodes, which we number from $k$.  For level $i \ge k$, the set $L_i$ consists of $2^{k+i}$ nodes, with the last level $\ell$ possibly having fewer than $m 2^\ell$ nodes.  There is an arbitrary bipartite graph connecting $L_i$ to $L_{i-1}$ with $d$ outgoing edges for each node in level $i$ and $2d$ incoming edges for each node $L_{i-1}$.  

 We now argue that $G$ is a stable network.  We make three observations about distances, which are critical in establishing that no node benefits by changing any of its outgoing edges.
  
    First, for any $0 \le i < k$, for any node $u$ in level $i$ and miner $v$, the distance  between  $u$ and $v$ is at most $2k - i + \delta_v$, where $\delta_v$ is the minimum, over all nodes in $L_0$, of the distance between the node and $v$.  This follows from the fact that any node in $L_k$ has a shortest path to every node in $L_0$; consequently, any node in $G_2$ has a path to $v$ by concatenating a subpath of length $k-i$ to the closest node in $L_k$, followed by a subpath of length $k$ to the node in $L_0$ that is closest to $v$, followed by a subpath of length $\delta_v$ to $v$.
  
  Second, for any $i \ge k$, for any node $u$ in level $i$ and miner $v$, the distance between $u$ and $v$ is exactly equal to $i + \delta_v$.  This holds since any node in $L_i$ has a path to $v$ by concatenating a subpath of length $i-k$ to an arbitrary node in $L_k$, 
  followed by a subpath of length $k$ to the node in $L_0$ that is closest to $v$
  followed by a subpath of length $\delta_v$ to $v$.
  
Finally, we note that for any leaf node $u$ and any miner $v$, the distance between $u$ and $v$ is at least $\ell + \delta_v$.  To complete the proof, we observe that for any $u$ in $G$ and any miner $v$, the distance between $u$ and $v$ is at most $\max\{i, 2k - i\} + \delta_v \le \ell + \delta_v$; consequently, replacing any out-edge with an out-edge to a leaf will not decrease its cost.  Therefore, $G$ is a stable network.
\end{proof}

    \subsection{Proof of Lemma~\ref{lem:no-stable-top}}
    \label{app:no-stable-top}
    \begin{lem}[LIFO and Global Ordering Tie-Breaking Instability for Large $m$]
            For all $m\geq 2d$, with \tiebreaks LIFO or global ordering, there exists no stable topology for $n\gg d$.
    \end{lem}
    \begin{proof}
        In this proof we essentially show that in a stable topology, 1.) there is a subset of miners who have the minimum score and all nodes must have all of their outgoing edges to this subset for the edge to be stable 2.) there are not enough miners in this subset so that all their outgoing edges are to each other, so some of their edges would be unstable.

        We know from Proposition~\ref{prop:first-d-1-stable}, any miner-stable topology must have that at least $d-1$ miners are connected to all miners (i.e., have the minimum score of $\frac{m-1}{m}$). We first argue that in a stable topology, all non-miners are also connected to some $d-1$ of these minimum-scored miners. If some non-miner is not, then in the next round it could connect to one of these miners it is not connected to and this connection will replace an existing connection (since less than $d-1$ of them have the minimum score). 
            
        To prove stability, we need to show that there does not exist an edge to a non-miner from some node which could be replaced by a new lower-scored edge to a non-miner in some round (i.e., there does not exist an unstable edge \textit{to} a non-miner). Since $n \gg d$, all non-miners cannot connect to all miners, so it must be that any stable edge from a miner to a non-miner must be to a non-miner with a score of 1 (for global ordering, these non-miners are the top-ranked ones), say there are $n'$ such non-miners. Equally, there are not enough edges for all non-miners to connect to each other. Consider a stable edge from non-miner $n_i$ to non-miner $n_j$. It must be that $n_i$ has a score of 1 (i.e., there does not exist a miner that can replace $n_j$ or another peer in the next round), and either $n_j$ has a score of 1 (otherwise a non-miner could get the lowest score in the next round and replace it) or all non-miners connect to $n_i$ (so there is no other out-going edge possible to replace $n_j$). This implies all non-miners with score $>1$ have all stable edges to miners, and thus at most 1 non-miner connects to all non-miners (with the $d$-th edge of these nodes) and this can change in any round, so there is no \textit{stable} edge to a non-miner with score $>1$. 

        Say a miner $m_i$ with score $>\frac{m-1}{m}$ has a stable edge to a miner $m_j$ with score $>\frac{m-1}{m}$, in the next round $m_i$ can connect to a miner it was not connected to before who in this round has score $\frac{m-1}{m}$ and replaces $m_j$ or other edge, thus the topology was not stable. We get that all miners with score $>\frac{m-1}{m}$ have all $d-1$ edges to miners with score $=\frac{m-1}{m}$ in a stable topology, so $n'$ is at most 1. So the single non-miner with a score $1$ would have only stable edges to miners, thus all stable edges from non-miners are to miners and all stable edges from miners are to miners. Since in some round a non-miner could have all miners connect to it, any stable edge to a miner must be to a miner with a score at most 1. 

        If there are no miners with a score of 1, then all miners with a score of $\frac{m-1}{m}$ must connect to each other with all their edges (needs to be $2d-1$ such miners), and all other miners must connect to these miners with their outgoing edges (max $d-1$ such miners). Thus, this is impossible.
            
        Say there are $m''$ miners with a score of 1, the rest must have score $\frac{m-1}{m}$ otherwise they would not connect to the score 1 miners. For a miner to have a score of 1, they must connect directly to all miners but 1, who they are 2 hops away from. So there are $m''= 2$ miners with score 1, so $m'=m-2$. For the $m'$ miners to form a clique, it must be that $m'\leq 2d-2$, thus given the bounds on $m$ we started it, we have that $2d-1< m \leq 2d+1$. For the $m'$ miners to connect to each other, we need $(m'-1)m'/2$ edges, and for the 2 miners to connect to them we need an additional $2m'$ edges, this must be equal to the number of edges of the $m$ miners thus $m(d-1)=\frac{m'(m'-1)}{2}+2m'$, substituting in $m'=m-2$ and simplifying, we get that we need
            $$(2d-2)=\frac{m'(m'+3)}{m'+2}$$
        to be satisfied. If $m=2d$, this gives us that $m'+2=m'+3$. If $m=2d+1$, we get $(m'-1)(m'+2)=m'(m'+3)$ which is only true for $m'=-1$. Thus, there are no conditions for stability.    

    \end{proof}

    \subsection{Proof of Lemma~\ref{lem:ran-no-stable}}
    \begin{lem}[FIFO and Random Tie-Breaking Instability for Large $n$]
            For all $m,d$, and $n>2d^2$ with \tiebreaks FIFO or random, there exists no stable topology.
        \label{app:ran-no-stable}
    \end{lem}
    \begin{proof}
            \noindent(Case 1: $m<d$) Assume there is a stable topology, this means all edges are stable and by Proposition~\ref{prop:only-stable-clique} the miners connect in a clique. The first observation is that, in a stable topology, all non-miners would connect to all miners. To see this, first, assume there is some non-miner $n_i$ who is not connected to all miners, there is a chance that in the next round, all miners connect to this $n_i$. Either this happens with $n_i$ making a connection to at least one new miner $m$, since miners have the minimum score, this connection will replace an existing connection to a non-miner. Or, this happens with some miner $m$ making a connection to $n_i$, in this round $n_i$ has the minimum non-miner score so it will replace an existing outgoing edge of $m$ to another non-miner if FIFO (or with some probability if random), since $m<d$. Thus, in a stable topology, all non-miners have an equal score of 1. 
            
            Non-miners who have all $d-1$ out-going edges to all miners have that those edges are stable since the miners are stable and have the lowest score. Since miners began the protocol with $d-1$ out-going edges, each miner must have maintained at least $d-1$ edges since you only drop an edge if you have $d$ edges. There are at least $d-1-m/2$ non-miners with incoming edges from a miner. If $m<d-1$, then non-miners who connect to at least 2 other non-miners (unless they are already connected to all non-miners which is not many since $n \gg d$). Thus take one of these non-miners, in the next round they connect to a non-miner that they were not already connected to, and since all non-miners have the same score, they replace one of their current non-miner connections with this new connection if FIFO (or with some probability, if random). Now consider $m=d-1$, some non-miners have all $d-1$ stable outgoing connections to all miners, thus at any point only one non-miner can connect to all non-miners (i.e. using the $d$-th edge of most non-miners). There is at least one miner with at most $\frac{m-1}{2}$ out-going connections, thus at least $d-1-\frac{m-1}{2}=d/2$ non-miners have at least one incoming connection from a miner. One of these non-miners is not connected to some other miner $m_i$, and in the next round could replace one of their existing connections to a non-miner with a connection to $m_i$ (with some probability). Thus there is always an unstable edge from the first $d-1$ out-going edges for some node.  

            % case 2
            \noindent(Case 2: $d\leq m < 2d$, FIFO or Random:) By Proposition~\ref{prop:only-stable-clique}, we know that for a topology to be stable, miners must connect in a clique which uses $\frac{m(m-1)}{2}$ edges. This leaves $m(d-1)-\frac{m(m-1)}{2}$ edges from the miners going out to non-miners. Assume that there exists at least one non-miner $n_i$ who is not connected to all miners. Node $n_i$ must have all outgoing edges to miners, otherwise, there is a miner it could connect to which would replace the edge since miners have the minimum score. Since $n_i$ is not connected to all miners, in the next round it could connect to some miner and this miner would (or could with some probability) replace an existing edge since they all have the same score. Now imagine all non-miners connect to all miners, it must be that all non-miners have all outgoing edges to all miners, otherwise, an outgoing edge to a non-miner can always be replaced (since there are not enough edges for non-miners to form a clique). Thus the only stable topology would be the unique case when the number of non-miners $n'$ is exactly such so that all non-miners connect to $d-1$ miners and have $m-(d-1)$ incoming connections from miners, thus
                $$n'(m-d+1)=m(d-1)-\frac{m(m-1)}{2}=\frac{m}{2}(2d-m-1)$$
            we get
                $$n = m+ n'=\frac{m}{2}\frac{(2m-2d+2)+(2d-m-1)}{(m-d+1)}=\frac{m}{2}\frac{m+1}{m-d+1}< \frac{dm}{m-d+1}<md<2d^2$$
            
            % case 3
            \noindent(Case 3: $m > 2d-1$, FIFO or Random:) By Proposition~\ref{prop:imposs-ran-stable}, there is no miner stable topology, so there is no stable topology.
            
    \end{proof}

    We note that if nodes could have less than $d-1$ outgoing edges, then there are cases where FIFO or random could lead to stable networks for smaller $m$. One such example is if $m=d-1$, we get the following stable topology: all miners connect in a clique and all non-miners have all stable $d-1$ outgoing edges to all miners. Since each miner is connected to all other nodes in the network, they would never gain more outgoing edges. All non-miners have just the $d$th edge to any other non-miner.

    \input{sections/app_additional_properties}

    \subsection{Proof of Proposition~\ref{prop:stable-inevitable}}

    \begin{prop}[Eventual Network Stability]
            If the number of miners $m < d$, given \tiebreak of Global-ordering or LIFO, the network will arrive at a stable topology.
            \label{app:stable-inevitable}
    \end{prop}
    \begin{proof}
        From Proposition~\ref{prop:eventual_clique} we get that the miners will eventually form a miner-stable topology which is a miner clique. Given this, in the remainder of the proof, we first argue that all edges involving miners will stabilize, and lastly that all edges between non-miners will stabilize.

        \textbf{1. $\forall i\leq m, e_{i,j}$ stabilizes for all $j$.} To ease our analysis, we present a process which defines a path from any miner-stable topology to all edges involving miners being stable. For LIFO, we define some arbitrary order over all nodes, note it is important non-miners choose their edges before the miners do. In both cases, if there are no such nodes that satisfy the process, the node chooses a random new edge.

        \noindent \textbf{Def. \textit{miner-stability-process}:} \\
        \indent For each round $r$:\\
        \indent\indent - Each non-miner chooses as their out-edge, the first miner it is not yet connected to.
        \indent\indent - Each miner chooses an their out-edge the first non-miner it is not connected to.

        We prove that $\forall i\leq m, \exists r$ s.t. $e_{i,j}$ is stable $\forall j$, via a strong induction proof.

        \textbf{Base case: (All of miner $m_1$'s edges will stabilize)} In the first round of the process, all non-miners $n_i$ not connected to  $m_1$, connect to it and thus $e_{1,i}=1$ with $n_i$ never dropping $m_1$ (miners have the smallest score and $d>m$). Assume there is some edge of $e_{1,j}$ which never stabilizes. This edge must be from $m_1$ to $n_j$ (otherwise $n_j$ would have connected to $m_1$ in some round), and so has value 1. For it not to be stable, at some point it must be dropped by $m_1$ at step 3. of some round $r$. If so, in round $r+1$ node $n_j$ would then make a stable edge to $m_1$ $\bot$.

        \textbf{Inductive step:} Assume that $\forall j' < j\leq m$ miner $m_{j'}$ is  stable at some round $r$. It must be that miner $m_j$ is connected to all nodes for $r'\geq r$, and note that if a non-miner connects to $m_j$, they never drop the connection as, again, miners have the smallest score and $d>m$. The proof follows similarly to the base case:

        Assume there is some edge of $e_{j,i}$ which never stabilizes. This edge must be from $m_j$ to $n_i$ (otherwise $n_i$ would have connected to $m_j$ in some round), and so has value 1. For it not to be stable, at some point it must be dropped by $m_j$ at step 3. of some round $r$. If so, in round $r+1$ node $n_i$ would then make a stable edge to $m_j$ $\bot$.

        We now have that all miner edges stabilize, what's left to show is that the non-miner edges will stabilize. 
        
        \textbf{2. $\forall i,j e_{i,j}$ stabilizes.} We've shown that all miners connect in a stable clique (have score of $\frac{m-1}{m}$, and all non-miners have stable connections to all miners (have score of $1$). Note for LIFO \tiebreak, all edges between non-miners are stable as they all have equal lowest-score which will never change. We just need to show that the non-miner edges for Global-Ordering \tiebreak stabilize. Again we define a stabilizing process:

        \noindent \textbf{Def. \textit{non-miner-stability-process}:} \\
        \indent For each round $r$:\\
        \indent\indent - Each non-miner who does not have $d-1$ stable edges, picks the smallest-indexed \\ \indent\indent ~~non-miner they are not connected to \\
        \indent\indent - All other non-miners then pick a random new node

        Again use a strong induction argument to prove all non-miners stabilize.

        \textbf{Base case: the smallest indexed non-miner $n_{m+1}$ stabilizes} Notice that in the first round of the process, all non-miners connect to $n_{m+1}$. Since it is smallest indexed non-miner, all incoming edges to it will not be replaced. Since it is connected to all nodes, and all incoming edges are stable, there are no other nodes, and will never be any other nodes, it could connect to as their $d$-th edge, so no outgoing edges will be dropped.

        \textbf{Inductive step:} Assume that $\forall  j' < j$ miner $n_{j'}$ is stable at some round $r$. Assume $n_j$ will never stabilize, this means there is some round $r'\geq r$ where $n_j$ will not gain any more stable edges. Assume in this round, some non-stable node $n_i$ connects to $n_j$. This edge will be stable as this node must already be connected to all $n_{j'}$ for $j'<j$, otherwise it wouldn't have chosen $j$, and all those connections are stable by the assumption, so there is no future edge that could win the tiebreak. If no new nodes pick $n_j$ as their outgoing edge, this means $n_j$ picked some node $n_i$ it was not connected to (otherwise it would have been stable) as its new edge. If $n_i$ has a smaller index than an existing edge, then it replaces that edge and stabilizes (as all incoming connections are stable). If $n_i$ does not replace an existing edge, this means all outgoing edges were stable. In every case we get a contradiction $\bot$.

     \end{proof}

==> sections/background.tex <==
\section{Background}
   [Add description of Perigee protocol]
